Antibody-Antigen Docking and Design via Hierarchical Equivariant Refinement

Computational antibody design seeks to automatically create an antibody that binds to an antigen. The binding affinity is governed by the 3D binding interface where antibody residues (paratope) closely interact with antigen residues (epitope). Thus, predicting 3D paratope-epitope complex (docking) is the key to finding the best paratope. In this paper, we propose a new model called Hierarchical Equivariant Refinement Network (HERN) for paratope docking and design. During docking, HERN employs a hierarchical message passing network to predict atomic forces and use them to refine a binding complex in an iterative, equivariant manner. During generation, its autoregressive decoder progressively docks generated paratopes and builds a geometric representation of the binding interface to guide the next residue choice. Our results show that HERN significantly outperforms prior state-of-the-art on paratope docking and design benchmarks.

==> temp.tex <==
\section{Simultaneous paratope folding and docking}

\textbf{Background}. When an antibody binds to an antigen, they form a joint structure called an antibody-antigen complex. Its binding interface is composed of a \emph{paratope} and an \emph{epitope}. A paratope is a sequence of antibody residues that are close to an antigen. They are usually located in the complementarity determining regions (CDRs) of an antibody. Similarly, an epitope is defined as the top $m$ antigen residues nearest to a paratope. Given a paratope sequence and the 3D structure of an epitope, our goal is to predict the 3D paratope-epitope complex by simultaneously folding and docking the paratope (Figure \ref{fig:interface}).

\textbf{Notations}. We denote an antigen as a sequence of residues $\vb = \vb_1\vb_2\cdots\vb_M$, with $m$ epitope residues $\vb_{e_1}\vb_{e_2}\cdots\vb_{e_m}$. Likewise, a paratope sequence is denoted as $\va = \va_1\cdots\va_n$. Each residue $\va_i$ can be either one of the 20 amino acids and consists of $n_i$ atoms $\set{\va_{i,1},\cdots,\va_{i,n_i}}$, with size $n_i \in [4, 14]$. 
The first four atoms in any residue correspond to its backbone atoms (N, C$_\alpha$, C, O), and the rest are its side chain atoms (C$_\beta$, C$_\gamma$, etc.).
The 3D coordinate of an atom $\va_{i,k}$ is denoted as $\vx(\va_{i,k}) \in \mathbb{R}^3$. 
%For ease of implementation, we pad all residues to 14 atoms by appending the C$_\alpha$ coordinates and use a mask vector $\vm_{i,k}$ for bookkeeping.
%For a binding interface residue $\va_i$, we denote $\vx(\va_{i,k})$ as $\vx_{i,k}$ to simplify notations. Note that $\va_i$ refers to a residue (amino acid) while $\va_{i,k}$ refers to one of its atoms.


\subsection{HSRN Model Overview}
We formulate binding interface design as a generative modeling task.
Given an antigen and its epitope $\va_1\cdots\va_m=\vb_{e_1}\cdots\vb_{e_m}$, a model needs to generate a paratope sequence $\va_{m+1}\cdots\va_{m+n}$ and its 3D structure so that they bind to the epitope. The overall generation process is illustrated in Figure~\ref{fig:paradigm}. In each generation step $t$, the model performs the following three actions.
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=0pt]
    \item Encode the current binding interface into a set of atom and residue vectors (section \ref{sec:hiermpn}).
    \item Predict the amino acid identity of the next paratope residue $\va_{m+t}$ based on its residue vector (section \ref{sec:generate}).
    \item Update the coordinate of all paratope atoms to accommodate the new paratope residue $\va_{m+t}$ and its atoms (epitope coordinates are fixed) (section \ref{sec:refinement}).
\end{enumerate}
The model repeats this process until all residues are generated. Importantly, HSRN represents a 3D structure by its atom coordinates because pairwise distance alone is not locally informative \cite{ingraham2019generative}. As a result, we must ensure that our structure refinement scheme is equivariant under epitope rotation and translation. 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/paradigm.pdf}
    \vspace{-15pt}
    \caption{Overview of the paratope generation process. Each circle is a residue whose amino acid identity is shown in capital letter and side chain shown as sticks. Residues with unknown identity are represented as a mixture of possible amino acids (pie charts). Dotted lines correspond to the edges in our hierarchical graph. We highlight atomic contacts between residues D and F (red circles) to illustrate the atom-level graph $\gG_\mathrm{atom}^{(t)}$. (a) In each step, HSRN encodes the current binding interface $\gG_\mathrm{res}^{(t)}, \gG_\mathrm{atom}^{(t)}$ into a set of residue and atom vectors and predicts the next residue Y. (b) It then updates the 3D coordinates of each residue/atom based on calculated forces $\vg_{ij}^{(t)}$. (c) Lastly, it constructs a new binding interface graph based on the new coordinates and repeats steps (a) and (b).}
    \label{fig:paradigm}
\end{figure*}

\subsection{Hierarchical Binding Interface Encoder}
\label{sec:hiermpn}

A binding interface is a complex structure that consists of an antigen, its epitope, and the binding paratope. Its representation should encode not only the interaction between paratope and epitope residues, but also the interaction between epitope residues and other interior antigen residues. Moreover, paratope-epitope interaction must be modeled at both residue and atomic resolutions. Two residues may appear to be far from each other in terms of C$_\alpha$ distance, but have strong atomic interactions (contacts) in the side chains (Figure~\ref{fig:paradigm}a). On the other hand, residue-level interactions are useful for predicting residue identities during generation. It provides a coarse-grained view of the binding interface that allows us to model long-range interactions efficiently. Since an antigen may contain over $10^3$ atoms, it is necessary to learn a hierarchical representation to model the complex interactions between two proteins at different scales.

To this end, we propose a protein encoder that represents a binding interface as a hierarchical graph, which consists of an antigen graph $\gG_\mathrm{ag}$, an atom-level interface graph $\gG_\mathrm{atom}$, and a residue-level interface graph $\gG_\mathrm{res}$. We encode the binding interface by a hierarchical message passing network (MPN) with three components.

\subsubsection{Antigen Encoder} 

We represent an entire antigen $\vb$ as a graph $\gG_\mathrm{ag}$, defined as the $K$ nearest neighbor graph of a point cloud of all its C$_\alpha$ atoms. Each residue $\vb_i$ is represented by its dihedral angles $\omega(\vb_i)$ calculated from backbone coordinates. Its amino acid features $\vf(\vb_i)$ indicate its polarity, hydropathy, volume, charge, and whether it is a hydrogen bond donor or acceptor.
Following \citet{ingraham2019generative}, we build a local coordinate frame for each residue $\vb_i$ and compute edge features $\vf(\vb_i, \vb_j)$ describing the distance, direction, and orientation between two residues $\vb_i$ and $\vb_j$. These features are rotation and translation invariant. The feature definitions are detailed in the appendix.

We encode $\gG_\mathrm{ag}$ by a standard MPN (architecture defined in the appendix). It learns a vector representation $\vh(\vb_i)$ for each antigen residue $\vb_i$ by
\begin{align}
    \vz(\vb_i) &= \vf(\vb_i) \oplus \omega(\vb_i) \\
    \set{\vh(\vb_i)} &= \MPN \big( \gG_\mathrm{ag}; \set{\vz(\vb_i)}, \set{\vf(\vb_i, \vb_j)} \big),
\end{align}
where $\oplus$ means vector concatenation and $\MPN(\cdot)$ is a message passing network with input node features $\set{\vz(\vb_i)}$ and edge features $\set{\vf(\vb_i, \vb_j)}$.

\subsubsection{Atom-level Interface Encoder}

The atom-level graph $\gG_\mathrm{atom}$ is defined as the $K$ nearest neighbor graph of a point cloud of all atoms $\set{\va_{i,k}}$ in the paratope and epitope. Each atom $\va_{i,k}$ is represented as a one-hot encoding $\vf(\va_{i,k})$ of its atom name (e.g., N, C$_\alpha$, C$_\beta$, O). Each edge $(\va_{i,k}, \va_{j,l})$ is represented as
\begin{equation}
   \vf(\va_{i,k}, \va_{j,l}) = \big(E_{\mathrm{pos}}(i - j),\;\mathrm{RBF}(\Vert \vx_{i,k} - \vx_{j,l} \Vert) \big),
\end{equation}
where the positional encoding $E_{\mathrm{pos}}(i - j)$ encodes the relative distance between two residues in the interface sequence and $\mathrm{RBF}(\cdot)$ encodes the distance between two atoms in a radial basis. We encode $\gG_\mathrm{atom}$ by another MPN which learns a vector representation $\vh(\va_{i,k})$ for each atom $\va_{i,k}$.
\begin{equation}
    \set{\vh(\va_{i,k})} = \MPN\big(\gG_\mathrm{atom}; \set{\vf(\va_{i,k})}, \vf(\va_{i,k}, \va_{j,l}) \big)
\end{equation}

\subsubsection{Residue-level Interface Encoder}

The residue-level graph $\gG_\mathrm{res}$ is defined as the $K$ nearest neighbor graph of all interface residues rooted at their C$_\alpha$ atoms. It is encoded by another MPN that operates on top of the antigen MPN and atom MPN. In particular, the initial representation $\vz(\va_i)$ is set differently for epitope and paratope residues:
\begin{equation}
    \vz(\va_i) = 
    \begin{cases}
        \big(\vh(\vb_{e_i}), \omega(\va_i), \sum_k \vh(\va_{i,k}) \big) & i \leq m \\
        \big(\vf(\va_i), \omega(\va_i), \sum_k \vh(\va_{i,k}) \big) & i > m \\
    \end{cases}
\end{equation}
For epitope residues $i \leq m$, their initial representation is the concatenation of three vectors: its dihedral angles $\omega(\va_i)$, $\vh(\va_{i,k})$ from the atom-level MPN, and $\vh(\vb_{e_i})$ from the antigen MPN. $e_i$ is the index of epitope residue $\va_i$ in the entire antigen sequence and $\vh(\vb_{e_i})$ captures the interaction between $\va_i$ and other antigen residues outside the binding interface. For paratope residues $i > m$, their initial representation uses the amino acid features $\vf(\va_i)$ instead. The residue-level MPN then applies message passing to derive the final residue representation $\vh(\va_i)$
\begin{equation}
    \set{\vh(\va_i)} = \MPN\big(\gG_\mathrm{res}; \set{\vz(\va_i)}, \set{\vf(\va_i, \va_j)} \big), 
\end{equation}
where $\vf(\va_i, \va_j)$ is defined in the same way as the antigen MPN.
In summary, the output of our hierarchical MPN is a set of residue representations $\vh(\va_i)$ and atom representations $\vh(\va_{i,k})$. The whole binding interface encoding process (involving three graphs) is denoted as 
\begin{equation}
    \set{\vh(\va_i)}, \set{\vh(\va_{i,k})} = \mathrm{HierMPN}(\gG_\mathrm{res}, \gG_\mathrm{atom}, \gG_\mathrm{ag})
\end{equation}

\section{Paratope generation}

Given epitope residues $\va_1\cdots\va_m$ and their 3D coordinates, HSRN generates paratope residues $\va_{m+1}\cdots\va_{n+m}$ autoregressively and updates the paratope 3D structure in each generation step. We propose to generate paratope residues and their 3D structure simultaneously because the 3D structure provide useful information for protein design \cite{ingraham2019generative,jin2021iterative}.

\subsubsection{Initial State}
At the outset, we need to predict the initial amino acid types and coordinates for paratope residues. We predict the paratope sequence length $n$ based on the epitope representations and guess the identity of each paratope residue
\begin{align}
    n &\sim \softmax \big(\mW_n \sum_{i=1}^m \vh(\vb_{e_i})\big) \\
    \vp^{(0)}_{m+i} &= \softmax\big(\mW_0 \vh^{(0)}(\va_{m+i}) \big) \\
    \vh^{(0)}(\va_{m+i}) &= \FFN(E_{\mathrm{pos}}(i))
\end{align}
where $E_{\mathrm{pos}}(i)$ is a positional encoding~\cite{vaswani2017attention} of the $i$\textsuperscript{th} paratope residue $\va_{m+i}$. $\vp^{(0)}_{m+i}[a]$ is the probability of residue $\va_{m+i}$ being amino acid type $a$. Since the amino acid of $\va_{m+i}$ is uncertain, its amino acid features in our hierarchical MPN are defined as the expectation of amino acid types: $\vf(\va_{m+i}) = \sum_a \vp^{(0)}_{m+i}[a] \vf(a)$. Compared to standard recurrent networks, this initial soft assignment allows our model to ``peak'' at the future residues without actually sampling them (c.f., pie chart nodes in Figure~\ref{fig:paradigm}).

Next, we need to predict the initial 3D coordinate of each paratope atom. Since the epitope coordinates are fixed, the initial prediction must be equivariant under epitope rotation and translation. To this end, HSRN predicts the pairwise distance between paratope and epitope C$_\alpha$ atoms based on the Euclidean distance of their residue representations
\begin{equation}
    \mD_{i,j} = \Vert \vh^{(0)}(\va_i) - \vh^{(0)}(\va_j) \Vert, 
\end{equation}
where $\vh^{(0)}(\va_j) = \vh(\vb_{e_j})$ for epitope residues ($j\leq m$) and $\vh^{(0)}(\va_i) = \FFN(E_{\mathrm{pos}}(i))$ for paratope residues ($i>m$).
Given this pairwise distance matrix $\mD\in \mathbb{R}^{(n+m)\times(n+m)}$, we can obtain their 3D coordinates by applying eigenvalue decomposition to the following Gram matrix
\begin{equation}
    \tilde{\mD}_{i,j} = 0.5(\mD_{i,1}^2 + \mD_{1,j}^2 - \mD_{i,j}^2), \quad \tilde{\mD} = \mU\mS\mU^\top
\end{equation}
where $\mS$ is a diagonal matrix whose first three columns $\mS_3$ contain the largest three eigenvalues. The coordinate of each residue $\va_i$ is calculated as 
\begin{equation}
    \tilde{\vx}^{(0)}_i = \mX_i, \quad \mX = \mU\sqrt{\mS_3}.
\end{equation}
Though the predicted coordinates $\set{\tilde{\vx}^{(0)}_i}$ retain the original distance $\mD$, they are not aligned with the given epitope. Moreover, they only characterize the backbone and we need to infer their side chain coordinates.
Therefore, we apply the Kabsch algorithm \cite{kabsch1976solution} to find a rigid body transformation $(\mR_k, \vt_k)$ that aligns the predicted epitope coordinates $\set{\tilde{\vx}^{(0)}_i}_{i \leq m}$ with the given epitope coordinates $\set{\vx(\vb_{e_i,k})}_{i \leq m}$ for each atom type $k\in [1,14]$
\begin{align}
    (\mR_k, \vt_k) &= \mathrm{Kabsch}\big(\set{\tilde{\vx}^{(0)}_i}_{i \leq m}, \set{\vx(\vb_{e_i,k})}_{i \leq m}\big) \\
    \vx^{(0)}_{m+j,k} &= \mR_k \tilde{\vx}^{(0)}_{m+j} + \vt_k \quad (1\leq j\leq n)
\end{align}
The resulting transformation $(\mR_k, \vt_k)$ is different for each atom type $k$ since the reference points $\set{\vx(\vb_{e_i,k})}_{i \leq m}$ are different. These coordinates will be updated in our structure refinement step even though they may be inaccurate initially.


\subsubsection{Residue Generation}
\label{sec:generate}

In each generation step $t$, the state of a binding interface $\gG_\mathrm{res}^{(t)}, \gG_\mathrm{atom}^{(t)}$ is defined by the current atom coordinates $\set{\vx_{i,k}^{(t-1)}}$ and residue identities $\set{\va_{m+i}}$. Since the epitope structure is fixed, we have $\vx_{i,k}^{(t)} = \vx(\vb_{e_i,k})$ for all $t\in [0,n]$. The identities of previous residues are already generated. To predict the identity of the next residue $\va_{m+t}$, we encode the current binding interface using a hierarchical MPN 
$$
    \set{\vh^{(t)}(\va_i)}, \set{\vh^{(t)}(\va_{i,k})} = \mathrm{HierMPN}_\theta(\gG_\mathrm{res}^{(t)}, \gG_\mathrm{atom}^{(t)}, \gG_\mathrm{ag})
$$
Note that we only need to run the antigen MPN once and reuse the outputs since the antigen graph $\gG_\mathrm{ag}$ is fixed. Based on the encoded vectors, we predict the amino acid type of the next residue $\va_{m+t}$ by
\begin{equation}
    \vp_{m+t} = \softmax\big(\mW_s \vh^{(t)}(\va_{m+t})\big)
\end{equation}
During training, we apply teacher forcing and set $\va_{m+t}$ to its true amino acid type. During testing, we sample an amino acid type $a \sim \vp_{m+t}$ and set $\va_{m+t}=\mathrm{one\_hot}(a)$. The future residues are still represented by their initial probability vectors $\vp_{*}^{(0)}$ since the generation process is autoregressive.

\textbf{Side chain masking}. In the beginning, we set the mask of each paratope residue $\va_{m+i}$ as $\vm_{m+i,k}^{(0)}= \mathbb{I}[k \leq 4]$ since its residue identity is unknown and all amino acids have four backbone atoms. When $\va_{m+t}$ is generated, its mask vector $\vm_{m+t,k}^{(t)}$ is updated based on its predicted amino acid type. The 3D coordinates of its side chain atoms remain as their initial values until $\va_{m+t}$ is generated. They do not provide any information about the residue type until step $t+1$.

\subsubsection{Hierarchical Structure Refinement}
\label{sec:refinement}

After the residue generation step, we need to update the all paratope coordinates to accommodate changes caused by $\va_{m+t}$. It is important to update the global 3D structure since the new paratope residue will affect the position of existing paratope atoms through physical forces. Moreover, the 3D structure update step must be \emph{equivariant} because the coordinates of epitope residues are given as inputs and they can be rotated and translated arbitrarily.

Therefore, we propose an equivariant update scheme by modeling the \emph{forces} between atoms. For backbone C$_\alpha$ atoms ($k = 1$), the strength of the force from atom $\va_{j,1}$ to $\va_{i,1}$ is calculated based on their residue-level representation
\begin{equation}
    \vg_{i,j}^{(t)} = \max\big\{\Delta - d_{ij}^{(t)}, \FFN\big(\vh^{(t)}(\va_i), \vh^{(t)}(\va_j) \big)\big\} \label{eq:force}
\end{equation}
where $d_{ij}^{(t)}$ is the current distance between atoms $\va_{i,1},\va_{j,1}$ and $\Delta=3.8\text{\AA}$ is the minimal distance allowed for two C$_\alpha$ atoms. This scheme prevents two atoms from clashing after applying the force.
We then update the C$_\alpha$ atom coordinates of each paratope residue by averaging the pairwise forces
\begin{equation}
    \vx_{i,1}^{(t)} = \vx_{i,1}^{(t-1)} + \frac{1}{n} \sum_{j\neq i} \vg_{i,j}^{(t)}(\vx_{i,1}^{(t-1)} - \vx_{j,1}^{(t-1)}) \label{eq:coord1}
\end{equation}
Following the proof from \citet{satorras2021n}, it is easy to show that Eq.(\ref{eq:coord1}) is equivariant under epitope rotation and translation.
For other atoms types ($k\neq 1$), the force from atom $\va_{j,l}$ to $\va_{i,k}$ is calculated from their atom-level representations $\vh^{(t)}(\va_{i,k})$ and $\vh^{(t)}(\va_{j,l})$
$$
    \vg_{ik, jl}^{(t)} = \max\big\{\delta - d_{ik,jl}^{(t)}, \FFN\big( \vh^{(t)}(\va_{i,k}), \vh^{(t)}(\va_{j,l}) \big)\big\}
$$
To prevent clashing, we truncate the force term if the current atom distance $d_{ik,jl}^{(t)}$ is less than the Van der Waals radius $\delta$. Similarly, we update the atom coordinates by applying all the pairwise forces
\begin{equation}
    \vx_{i,k}^{(t)} = \vx_{i,k}^{(t-1)} + \frac{1}{n} \sum_{j,l} \vg_{ik, jl}^{(t)} (\vx_{i,k}^{(t-1)} - \vx_{j,l}^{(t-1)}) \label{eq:coord2}
\end{equation}
In practice, we found this update scheme consumes prohibitively large memory due to the large number of atoms. For computational efficiency, we only model the force between atoms within the same residue, i.e. $\vg_{ik, jl}^{(t)} = 0, \forall j \neq i$. In summary, the first C$_\alpha$ update step models the global 3D structure refinement and the second atom update step focuses on the local side chain arrangement.

\subsubsection{Training Loss}
Our training loss $\gL = \gL_\mathrm{init} + \gL_\mathrm{seq} + \gL_\mathrm{struct}$ contains three terms. The initial prediction loss is defined as
$$
    \gL_\mathrm{init} = \sum_i \ell_{ce}(\vp^{(0)}_{m+i}, \va_{m+i}) + \sum_{i,j} (\mD_{i,j} - \Vert \vx_{i,1} - \vx_{j,1} \Vert)^2
$$
where $\ell_{ce}$ is the cross entropy loss. The sequence generation loss is defined as
$
    \gL_\mathrm{seq} = \sum_t \ell_{ce}(\vp_{m+t}, \va_{m+t})
$.
To compute the structure prediction loss, we first calculate the mean square error between predicted dihedral angles and their ground truth in each generation step
$
     \mathcal{L}_a^{(t)} = \sum_i \Vert \omega^{(t)}(\va_i) - \omega(\va_i)\Vert^2
$.
Next, we compute the pairwise distance between all atoms in the binding interface and calculate the distance loss for every generation step
\begin{equation}
    \mathcal{L}_{ik,jl}^{(t)} = \sum_{i,j,k,l} \ell_{h}(\Vert \vx_{i,k}^{(t)} - \vx_{j,l}^{(t)} \Vert^2, \Vert \vx_{i,k} - \vx_{j,l} \Vert^2)
\end{equation}
where $\ell_{h}$ is the Huber loss. We then accumulate the pairwise distance loss across all generation steps
\begin{equation}
    \gL_\mathrm{struct} = \sum_{t=1}^n \bigg(\mathcal{L}_a^{(t)} + \sum_{i,j,k,l} \vm_{i,k}^{(t)}\vm_{j,l}^{(t)} \mathcal{L}_{ik,jl}^{(t)}\bigg),
\end{equation}
where $\vm_{i,k}^{(t)}=0$ if a side chain atom $k$ is not created at time step $t$. For training stability, we add stop-gradient operators to the intermediate coordinates during back-propagation. 
